A Compressed Sensing Wire-Tap Channel

A multiplicative Gaussian wire-tap channel inspired by compressed sensing is studied. Lower and upper bounds on the secrecy capacity are derived, and shown to be relatively tight in the large system limit for a large class of compressed sensing matrices. Surprisingly, it is shown that the secrecy capacity of this channel is nearly equal to the capacity without any secrecy constraint provided that the channel of the eavesdropper is strictly worse than the channel of the intended receiver. In other words, the eavesdropper can see almost everything and yet learn almost nothing. This behavior, which contrasts sharply with that of many commonly studied wiretap channels, is made possible by the fact that a small number of linear projections can make a crucial difference in the ability to estimate sparse vectors.

==> sections/introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
Following Shannon's theory in 1949 of information-theoretic secrecy~\cite{shannon49}, Wyner introduced the wiretap channel in 1975~\cite{wyner}. In the wiretap setting, a sender Alice wishes to communicate a message to a receiver Bob over a main channel but her transmissions are intercepted by an eavesdropper Eve through a secondary wiretap channel. The present paper analyzes a multiplicative Gaussian wiretap channel inspired by compressed sensing. The input to the channel is a $p$-length binary vector. The channel output is a linear transform of the input after it has first been corrupted by multiplicative white Gaussian noise. We analyze the setting where Bob and Eve observe different linear transforms characterized by two different channel matrices.

Secrecy via compressed sensing schemes has received little attention from an information-theoretic viewpoint. In prior work, authors consider using a sensing matrix as a key (unknown to the
eavesdropper) for both encryption and compression~\cite{rachlin2009secrecy}. Privacy via compressed sensing and linear programming decoding was explored in~\cite{cynthia07privacy}. By contrast, this paper assumes that the sensing matrices are known (non-secret); as a special case, Eve's sensing matrix might correspond to a subset of the rows of Bob's channel matrix. Our analysis shows that certain channel matrices, inspired by compressed sensing, allow for secrecy rates that are nearly equal to the main channel capacity even if Eve's capacity is large.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Channel Model}

\begin{figure}[t]
\centering
\includegraphics[scale=0.48]{figures/wiretap_channel}
\caption{ {{ \emph{(Multiplicative Gaussian Wiretap Channel)} For each block length $n$, Alice transmits a sequence of $n$ binary valued support vectors $\bX \in \{0,1\}^{p}$ over a main channel characterized by a matrix transform so that Bob receives $\bY = A_bW\bX$. The eavesdropper Eve receives $\bZ = A_eW\bX$.}} } \label{fig:WiretapChannel}
\end{figure}

Outlined in Fig.~\ref{fig:WiretapChannel}, the multiplicative Gaussian wiretap channel with binary vector input is characterized by
\begin{align}
\bY & = A_b W \bX, \\
\bZ & = A_e W \bX,
\end{align}
where $\bX \in \{0,1\}^{p}$ is the transmitted signal, and $\bY \in \mathbb{R}^{m_b}$, $\bZ \in \mathbb{R}^{m_e}$ are the received real-valued signals at the legitimate user and eavesdropper, respectively. A related channel model in~\cite{liu07} also involves a wire-tap setting with binary input and real-valued output. The dimensions of the channel satisfy $0 \leq m_e < m_b < p/2$. The linear mixing parameters, matrices $A_b \in \mathbb{R}^{m_b \times p}$ and $A_e \in \mathbb{R}^{m_e \times p}$, are fixed and known to all parties. The randomness of the channel is derived from $W \in \mathbb{R}^{p \times p}$, a diagonal matrix whose values are i.i.d.~Gaussian random variables with mean zero and variance one. The channel is assumed to be memoryless between channel uses. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Secrecy Capacity}
%Alice selects a message $S_n \in [1: N_n]$ and wishes to communicate reliably with Bob while keeping the message secret from Eve. A $(N_n, n)$ secrecy code for the multiplicative wiretap channel consists of the following: (1) A message set $[1:N_n]$; (2) A randomized encoder that generates a codeword $\bX^{n}(S_n)$, $S_n \in [1:N_n]$, according to $P_{\bX^{n}|S_n}$; (3) A decoder that assigns a message $\hat{S}_n(\bY^{n})$ to each received sequence $\bY^{n} \in \mathcal{Y}^{n}$. A sequence of $(N_n,n)$ secrecy codes is said to achieve a {\em normalized} secrecy rate $R_s$ if 
%%The message $S_n$ is a random variable with entropy satisfying
%\begin{align}
%\lim_{n \rw \infty} \textstyle \frac{1}{n} H(S_n) = p R_s
%\end{align}
%and
%\begin{align}
%\lim_{n \rw \infty} \Pr[ \hat{S}_n(\bY^{n}) \ne S_n] =0.
%\label{eqn:codereliable}
%\end{align}
%A secrecy code is secret if the information leakage rate tends to zero as block length $n \rw \infty$,
%\begin{align}
%\lim_{n \rw \infty} \frac{I(\bZ^{n} ; S_n)}{n} = 0.
%\label{eqn:codesecret}
%\end{align}
%Note that this leakage rate is not normalized by $p$. A normalized rate $R$ is achievable if there exists a sequence of $(2^{npR}, n)$ secrecy codes satisfying both Eqn.~\eqref{eqn:codereliable} and Eqn.~\eqref{eqn:codesecret}. The secrecy capacity $C_s$ is the supremum over all achievable rates.

%%\begin{definition}
%%A normalized secrecy rate $R$ is achievable for the multiplicative Gaussian wiretap channel if there exists a sequence of $(N_n,n)$ secrecy codes for which:
%%\begin{align}
%%\lim_{n \rw \infty} {\textstyle \frac{1}{n} } H(S_n)& =p R\\
%%\lim_{n \rw \infty}\Pr[ \hat{S}_n(\bY^{n}) \ne S_n] &=0\\
%%\lim_{n \rw \infty} {\textstyle \frac{1}{n} } I(\bZ;S_n)) & =0.
%%\end{align}
%%The first two conditions guarantee that Alice can communicate reliably with Bob at rate $pR$. The third condition guarantees that the leakage rate $I(\bZ;S_n)$  
%%%\begin{itemize}
%%%\item $$\lim_{n \rw \infty} {\textstyle \frac{1}{n} }\log(N_n) =p R$$
%%%\end{itemize}
%%\end{definition}


Alice selects a message $S_n \in [1 : 2^{npR}]$, where $R$ represents a normalized rate, and wishes to communicate reliably with Bob while keeping the message secret from Eve. A $(2^{npR}, n)$ secrecy code for the multiplicative wiretap channel consists of the following: (1) A message set $[1:2^{npR}]$; (2) A randomized encoder that generates a codeword $\bX^{n}(S_n)$, $S_n \in [1:2^{npR}]$, according to $P_{\bX^{n}|S_n}$; (3) A decoder that assigns a message $\hat{S}_n(\bY^{n})$ to each received sequence $\bY^{n} \in \mathcal{Y}^{n}$. The message $S_n$ is a random variable with entropy satisfying
\begin{align}
\lim_{n \rw \infty} \frac{H(S_n)}{np} = R.
\end{align}
A secrecy code is reliable if
\begin{align}
\lim_{n \rw \infty} \Pr[ \hat{S}_n(\bY^{n}) \ne S_n] =0.
\label{eqn:codereliable}
\end{align}
A secrecy code is secret if the information leakage rate tends to zero as block length $n \rw \infty$,
\begin{align}
\lim_{n \rw \infty} \frac{I(\bZ^{n} ; S_n)}{n} = 0.
\label{eqn:codesecret}
\end{align}
Note that this leakage rate is not normalized by $p$. A normalized rate $R$ is achievable if there exists a sequence of $(2^{npR}, n)$ secrecy codes satisfying both Eqn.~\eqref{eqn:codereliable} and Eqn.~\eqref{eqn:codesecret}. The secrecy capacity $C_s$ is the supremum over all achievable rates.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Outline}

To analyze the secrecy capacity $C_s$, we first develop bounds as a function of the channel matrices $A_b$ and $A_e$. We then analyze these bounds for certain random matrices in the large system limit where $m_b/p \rw \rho_b$ and $m_e/p \rw \rho_e$ as $p \rw \infty$ for fixed constants $0 \le \rho_e \le \rho_b \le 1/2$. Lower bounds on the secrecy capacity, corresponding to Wyner's coding strategy for discrete memoryless channels are developed in Section~\ref{sec:LB}. Corresponding upper bounds are derived in Section~\ref{sec:UB}. Section~\ref{sec:UB2} provides an improved upper bound under a certain encoding constraint on Alice. Proofs are given in Section~\ref{sec:proofs}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Notations}
For a matrix $A \in \mathbb{R}^{m \times p}$ and vector $\bx\in
\{0,1\}^p$, we use $A(\bx)$ to denote the matrix formed by concatenating
the columns indexed by $\bx$, and we use $A(i)$ to denote the $i$th column of $A$. Also, we use $\mathcal{X}_k^p$ to denote the set of all binary vectors $\bx \in \{0,1\}^p$ with
exactly $k$ ones.  We use $H_2(x) = -x \log x - (1-x) \log(1-x)$ to denote binary the binary entropy function. We use $\log$ to denote the logarithm with base two and $\ln$ to denote the logarithm with the natural base. 

==> sections/proofs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proofs}\label{sec:proofs}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem~\ref{thm:LB1}}\label{sec:thm-LB1-proof}

Let $U = \bX$ where $\bX$ is distributed uniformly over $\mathcal{X}_{m_b-1}^p$.  Since $A_b$ is fully linearly independent, the probability that $\bY$ is in the range space of $A_b(\tilde{\bx})$ for any $\tilde{\bx} \in \mathcal{X}_{m_b-1}^p$ not equal to the true vector $\bX$ is equal to zero. Thus, $H(\bX|\bY) =0$ and
\begin{align}
I(U;\bY)= I(\bX;\bY) = H(\bX) = \textstyle \log {p \choose m_b -1}. \label{eq:hY1}
\end{align}

Next, since $A_e$ is fully linearly independent and the number of nonzero values in $\bX$ is strictly greater than the rank of $A_e$, it can be verified that both $\bZ$ and $\bZ|\bX$ have probability densities. (Note that the condition $m_b > m_e$ is critical here, since $\bZ$ does not have a density otherwise.) %, since $Z_{m_e}| Z_1, Z_2,\cdots,Z_{m_e-1}$ is distributed over a finite number of possibilities). 
Thus we can write
\begin{align}
I(U;\bZ) = I(\bX;\bZ) = h(\bZ) - h(\bZ|\bX) \label{eq:hZ1}
\end{align}
where $h(\cdot)$ denotes differential entropy (see e.g. \cite{elementsofIT}). The entropy $h(\bZ)$ can be upper bounded as
\begin{align}
h(\bZ) & \le \max_{\tilde{\bZ} \; : \; \bE[  \tilde{\bZ} \tilde{\bZ}] = \bE[\bZ \bZ^T]} h(\tilde{\bZ}) \nonumber \\
&\le \textstyle \frac{1}{2} \log \big( (2 \pi e)^{m_e} \det( \bE[ \bZ \bZ^T])\big) \label{eq:hbZ2}\\
&= \textstyle \frac{1}{2} \log \big( (2 \pi e \, (\frac{m_b-1}{p}))^{m_e} \det( A_e A_e^T)\big) \label{eq:hZ2}
\end{align}
where \eqref{eq:hbZ2} follows from the fact that the Gaussian distribution maximizes differential entropy and \eqref{eq:hZ2} follows from the fact that
\begin{align}
\bE[ \bZ \bZ^T] = \textstyle\frac{m_b-1}{p} A_e A_e^T.
\end{align}

The conditional entropy $h(\bZ|\bX)$ is given by
\begin{align}
h(\bZ|\bX) &=  \textstyle \bE \left[ \frac{1}{2} \log\big( (2 \pi e)^{m_e} \det(A_e(\bX) A_e(\bX)^T)\big) \right]  \label{eq:hZ3}
\end{align}
where we used the fact that, conditioned on any realization $\bX=\bx$, $\bZ$ is a (non-degenerate) Gaussian random vector with covariance matrix $A_e(\bx) A_e(\bx)^T$. Combining \eqref{eq:hY1}, \eqref{eq:hZ1}, \eqref{eq:hZ2}, and \eqref{eq:hZ3} with the expression of the secrecy capacity given in \eqref{eq:CsThm} completes the proof of Theorem~\ref{thm:LB1}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem~\ref{thm:LB2}}\label{sec:thm-LB2-proof}
%If $\bA\in \mathbb{R}^{m \times p}, m \le p$ is a random matrix whose elements are i.i.d.~$\mathcal{N}(0,1)$, then $\det(\bA \bA^T)$ is equal in distribution to $\prod_{i=1}^m Z_i$ where $Z_i \sim \chi^2_{p-i+1}$ are independent (see e.g. \cite[Theorem 3.2.15]{Muirhead}). Using the fact that $\bE[ \log \chi^2_i] = \log 2 + \psi(i/2)$ and the linearity of expectation, allows us to compute the expectation of the right hand side of \eqref{eq:CsLB1} with respect to the distribution on $\bA_e$.

It is straightforward to show that $\bA_e$ is fully linearly independent with probability one. Since the secrecy rate is bounded, it thus follows from Theorem \ref{thm:LB1} and the linearity of expectation that
\begin{align}
\bE[C_s] &\ge \textstyle \frac{1}{p}  \log{p \choose m_b -1} -  \frac{m_e}{2p}\log \big( \frac{m_b-1}{p}\big) \nonumber \\
& -\frac{1}{2p} \bE\big[ \log \det(\bA_e \bA_e^T)\big] \nonumber\\
&+%{\textstyle \frac{1}{2p}}
 \sum_{\bx \in \mathcal{X}^p_{m_b-1}} \textstyle {\textstyle \frac{1}{ {p \choose m_b -1}2 p}} \bE\big[ \log \det\left( \bA_e(\bx)\bA_e(\bx)^T\right)\big]. \label{eq:ECs_proof}
\end{align}
Using well known properties of random Gaussian matrices (see e.g. \cite[pp. 99-103]{Muirhead}) shows that
%Next, if $\bA\in \mathbb{R}^{m \times p}, m \le p$ is a random matrix whose elements are i.i.d.~$\mathcal{N}(0,1)$, then $\det(\bA \bA^T)$ is equal in distribution to $\prod_{i=1}^m Z_i$ where $Z_i \sim \chi^2_{p-i+1}$ are independent (see e.g. \cite[Theorem 3.2.15]{Muirhead}). Since $\bE[ \log \chi^2_i] = \log 2 + \psi(i/2)$, we conclude that
%then it is well known (see e.g. \cite[Theorem 3.2.15]{Muirhead}) that $\bE \big[ \log \det(\bA \bA^T) ] = m \log2 + \sum_{i=1}^{m} \psi({\textstyle \frac{p-i+1}{2}})$. Thus,
\begin{align*}
\bE \big[ \log \det(\bA_e \bA_e^T) ] &= m_e  + \log e \sum_{i=1}^{m_e} \psi({\textstyle \frac{p-i+1}{2}})\\
\bE \big[ \log \det(\bA_e(\bx) \bA_e(\bx)^T) ]& = m_e  + \log e\sum_{i=1}^{m_e} \psi({\textstyle \frac{m_b-i}{2}})
\end{align*}
where the second equality holds for every $\bx \in \mathcal{X}^p_{m_b-1}$. Plugging these expressions into \eqref{eq:ECs_proof} completes the proof. %the proof of Theorem~\ref{thm:LB2}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem~\ref{thm:LB3}}\label{sec:thm-LB3-proof}

Since $\bA_e$ is fully linearly independent with probability one, it is sufficient to consider the asymptotic behavior of the bound in Theorem~\ref{thm:LB1}. If $\bX$ is a random vector distributed uniformly over $\mathcal{X}_{m_b-1}^p$ then $\bA_e\bA_e^T$ and $\bA_e(\bX)\bA_e(\bX)^T$ are $m_e \times m_e$ Wishart matrices with $p$ and $m_b-1$ degrees of freedom respectively. Using Lemma~\ref{lem:det_concentration} in the Appendix gives
\begin{align*}
\lim_{p \rw \infty}  \textstyle \frac{1}{p} \log \det (\frac{1}{p} \bA_e \bA^T_e)& = \mu(\rho_e)\\
\lim_{p \rw \infty}  \textstyle \frac{1}{p } \log \det (\frac{1}{m_b-1} \bA_e(\bX) \bA^T_e(\bX)) &=  \rho_b\,  \mu(\rho_e/\rho_b) 
\end{align*}
almost surely where $\mu(r) = (1-r) \ln \big( {\textstyle \frac{1}{1-r}}\big) -r\log e$. Thus,
%Since the expectation of $\frac{1}{m_b}\log \det (\frac{1}{m_b} \bA(\bX)\bA_e(\bX)^T)$ with respect to both $\bA$ and $\bX$ is bounded uniformly for all $p$ (see the proof of Theorem~\ref{thm:LB2}), we can replace the random vector $\bX$ with the weighted sum over all $\mathcal{X}_{m_b-1}^p$. Thus%  taking expectation with respect to $\bX$ does not affect the convergence. Thus
\begin{align}
\lim_{p \rw \infty} & \bigg[\textstyle  \frac{m_e}{p} \log\big(\frac{m_b-1}{p}\big)  \frac{1}{p} \log \det(\bA_e \bA_e^T)  \nonumber\\
&-   \sum_{\bx \in \mathcal{X}^p_{m_b-1}} \textstyle {\textstyle \frac{1}{ {p \choose m_b -1}  p}} \log \det ( \bA_e(\bx) \bA_e(\bx)^T) \bigg]  \nonumber \\
&= \lim_{p \rw \infty}  \bigg[\textstyle  \frac{m_e}{p} \log\big(\frac{m_b-1}{p}\big)  \frac{1}{p} \log \det(\bA_e \bA_e^T)  \nonumber\\
&\quad -   \textstyle {\textstyle \frac{1}{ p}} \log \det ( \bA_e(\bX) \bA_e(\bX)^T) \bigg]  \label{eq:converg_X} \\
&= \mu(\rho_b) - \rho_b \,\mu(\rho_e/\rho_b)  \nonumber \\
& = (1 - \rho_e) \log\big(\textstyle\frac{1} {1 - \rho_e} \big) - (\rho_b - \rho_e) \log\big(\textstyle \frac{\rho_b}{\rho_b - \rho_e}\big) \label{eq:limLB3}
\end{align}
almost surely where the substitution in  \eqref{eq:converg_X} is justified by the fact that the expectation of $\frac{1}{m_b}\log \det (\frac{1}{m_b} \bA(\bX)\bA_e(\bX)^T)$ with respect to both $\bA$ and $\bX$ is bounded uniformly for all $p$ (see the proof of Theorem~\ref{thm:LB2}).
%
% %$for any fixed sequence of vectors $\bx \in \mathcal{X}_{m_b-1}^p$ where
%\begin{align}
%%\mu(\rho) = (1-\rho) \log \big( {\textstyle \frac{1}{1-\rho}}\big) - \rho. %(1-1/\rho ) \log(1-\rho) - 1
%\mu(r) = (1-r) \log \big( {\textstyle \frac{1}{1-r}}\big) -r. \label{eq:mu}
%%\begin{cases}
%%0, & \text{\normalfont if $\rho = 0$}\\
%%(1-\rho) \log \big( {\textstyle \frac{1}{1-\rho}}\big) - \rho,  & \text{\normalfont if $0<\rho <1$}\\
%%-1, & \text{\normalfont if $\rho = 1$}\\
%%\end{cases}.
%\end{align}

Combining \eqref{eq:limLB3} with the well known fact that %Also, using well known approximation
\begin{align}
\lim_{p \rw \infty}  \textstyle \frac{1}{p} \log {p \choose m_b-1} = H_2(\rho_b) \label{eq:H_bin}
\end{align}
completes the proof of Theorem~\ref{thm:LB3}.

%If $\bA\in \mathbb{R}^{m \times p}$ is a random matrix whose elements are i.i.d.~with mean zero and variance one and if $m = \lfloor \rho p \rfloor$ for some $\rho \in (0,1)$, then the empirical spectral distribution of $\frac{1}{p} \bA \bA^T$ converges almost surely to a nonrandom limit known as the Marcenko-Pastur law (see e.g. \cite{Salo06}). It can be verified that almost sure convergence of the spectral distribution on $\frac{1}{p} \bA \bA^T$ implies almost sure convergence of the right hand side of \eqref{eq:CsLB1} to a nonrandom limit. This value of this limit can be computed either by direct integration with respect to the Marcenko-Pasture law, or by studying the asymptotic behavior of \eqref{eq:LB2}. See \cite{Salo06} for more details.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem~\ref{thm:UB1}}\label{sec:thm-UB1-proof}

Let $K = \sum_{i=1}^p X_i$ denote the number of ones in $\bX$. Then,
\begin{align}
I(\bX; \bY) &= I(\bX;\bY | K) + I(\bY; K) \label{eq:IbA} \\
&\le I(\bX;\bY| K) + \log p \label{eq:IbB} \\
& \le \max_{0 \le k \le p} I(\bX;\bY|K=k) + \log p  \label{eq:IbC}
\end{align}
where \eqref{eq:IbA} follows from the chain rule for mutual information, \eqref{eq:IbB} follows from the fact that $I(\bY;K) \le H(k) \le \log p$, and \eqref{eq:IbC} follows from expanding the term $I(\bX;\bY|K)$. If we define
\begin{align*}
c(k) = \max_{\bX \in \mathcal{X}_k^p} I(\bX;\bY)
\end{align*}
then we have
\begin{align}
 \max_{\bX} I(\bX;\bY) & \le \max_{0 \le k \le p} c(k) + \log p. \label{eq:Iboundmax}%\\
% & \le \max \big({\textstyle \log{ p \choose m_b -1}}, \max_{ m_b \le k \le k} c(k) \big)  + \log p \nonumber
\end{align}
To complete the proof, we split the maximization over $k$ into two cases. For $ 0 \le k < m_b$ we use the simple bound%the first case, we use%.use the upper bound
\begin{align*}
\max_{0 \le k < m_b} c(k) \le \max_{\bX \in \mathcal{X}_k\, : \; 0 \le k < m_b} H(\bX) = {\textstyle \log {p \choose m_b-1}}.
\end{align*}
For $m_b \le k \le p$ we use the following lemma.

\begin{lemma}\label{lem:ckbound2}
If $m_b \le k \le p$, then $c(k) \le \tilde{c}(k)$ where $\tilde{c}(k)$ is given in \eqref{eq:Ctilde}.
\end{lemma}
\begin{proof}
Let $\bX$ have any distribution on $\mathcal{X}_k^p$ where $m_b \le k \le p$. Since $A_e$ is fully linearly independent, both $\bY$ and $\bY|\bX$ have probability densities and we can write
\begin{align}
I(\bX;\bY) = h(\bY) - h(\bY|\bX) \label{eq:Inf1}
\end{align}
where $h(\cdot)$ denotes differential entropy (see e.g. \cite{elementsofIT}). The entropy $h(\bY)$ can be upper bounded as
\begin{align}
h(\bY) & \le \max_{\tilde{\bY} \; : \; \bE[ \| \tilde{\bY} \|^2] = \bE[\|\bY\|^2]} h(\tilde{\bY})\nonumber \\
& =\textstyle \frac{m_b}{2} \log\big( 2 \pi e \,\frac{1}{m_b} \bE[ \| \bY\|^2] \big) \label{eq:hB1}\\
& \le \max_{1\le i \le p}  \textstyle \frac{m_b}{2} \log\big( 2 \pi e\textstyle \frac{k}{m_b} \| A_b(i)\|^2 \big) \label{eq:hB2}
\end{align}
where \eqref{eq:hB1} follows from the fact that an isotropic Gaussian vector maximizes differential entropy, and \eqref{eq:hB2} follows from the fact that
\begin{align*}
\bE[ \|\bY\|^2]& = \bE \big[  \bE[ \| \bY \|^2 | \bX] \big]\\
& \le \max_{\bx}  \bE[ \| \bY \|^2 | \bX=\bx] \\
&=  \max_{\bx}  \tr\big(A_b(\bx) A_b(\bx)^T\big)\\
&\le  \max_{1 \le i \le p} k  \| A_b(i)\|^2.
\end{align*}


The conditional entropy $h(\bY|\bX)$ is lower bounded by
\begin{align}
h(\bY|\bX) &=  \textstyle \bE \left[ \frac{1}{2} \log\big( (2 \pi e)^{m_b} \det(A_b(\bX) A_b(\bX)^T)\big) \right]
\nonumber \\
& \ge  \min_{\bx \in \mathcal{X}_k^p} \textstyle \frac{1}{2} \log\big( (2 \pi e)^{m_b}   \det(A_b(\bx) A_b(\bx)^T)\big)\label{eq:hB3}
\end{align}
where we used the fact that, conditioned on any realization $\bX=\bx$, $\bY$ is a (non-degenerate) Gaussian random vector with covariance matrix $A_b(\bx) A_b(\bx)^T$. Combining \eqref{eq:Inf1}, \eqref{eq:hB2} and \eqref{eq:hB3} completes the proof of Theorem~\ref{thm:UB1}.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem~\ref{thm:UB2}}\label{sec:thm-UB2-proof}

Since $\bA_e$ is fully linearly independent with probability one, it is sufficient to consider the asymptotic behavior of the bound in Theorem~\ref{thm:UB1}. The limit of the first term in the maximization is given by \eqref{eq:H_bin}. To evaluate the second term, we use the following technical lemmas whose proofs are given in the Appendices \ref{sec:tracebound-proof} and \ref{sec:detbound-proof}. %omitted due to space constraints

\begin{lemma}\label{lem:tracebound}
\begin{align}
\limsup_{p \rw \infty} \max_{1 \le i  \le p} \frac{1}{m_b}\|\bA_b(i)\|^2 \le 1
\end{align}
almost surely.
\end{lemma}

\begin{lemma}\label{lem:detbound}
If $k  \ge m_b$ and $k/p \rw \kappa$ where $\rho_b \le \kappa \le 1$, then
\begin{align}
\liminf_{p \rw \infty} \min_{\bx \in \mathcal{X}_k^p} \textstyle \frac{1}{p} \log \det (\frac{1}{k} \bA_b(\bx) \bA_b(\bx)^T) \ge   \kappa\, \mu(\rho_b/\kappa)
\end{align}
almost surely where $\mu(r) = (1-r) \log \big( {\textstyle \frac{1}{1-r}}\big) -r \log e$.%$\mu(x) = (1-1/x)\log(1-x) - 1$.
\end{lemma}

The convergence show in Lemmas \ref{lem:tracebound} and \ref{lem:detbound} leads immediately to  the following asymptotic upper bound on the term $\tilde{c}(k)$ defined in \eqref{eq:Ctilde}:
% to the second term in upper bound of Theorem Theorem~\ref{thm:UB1} gives
%
%We now prove that $H(\rho_b)$ is an asymptotic upper bound on the capacity. Let $k = \lceil \kappa\, p \rceil$. Since $\lim_{p \rw \infty} \frac{1}{p}\log{p \choose k} = H(\kappa)$, we have
%\begin{align}
%\limsup_{p \rw \infty} \textstyle \frac{1}{p} c(k) \le H(\kappa).
%\end{align}
%Also, if $\kappa > \rho_b$ then it follows from Lemmas \ref{lem:ckbound2}, \ref{lem:tracebound} and \ref{lem:detbound} that %shows that if $\kappa > \rho_b$, then
\begin{align*}
&\limsup_{p \rw \infty} \max_{m_b < k \le p}  \textstyle \frac{1}{p} \tilde{c}(k) \\
&\le \max_{\rho_b \le \kappa \le 1} \textstyle \frac{1}{2} \big[ \rho_b \log e - (\kappa - \rho_b) \log \big( \frac{\kappa}{\kappa - \rho_b }\big)\big] \\
& = \textstyle \frac{1}{2}\rho_b \log e
\end{align*}
almost surely. Since $H_2(\rho_b)> \frac{1}{2}\rho_b  \log e$ for all $\rho_b \in (0,1/2)$, we conclude that the asymptotic capacity is upper bounded by $H_2(\rho_b)$. The achievable strategy outlined in the proof of Theorem~\ref{thm:LB1} shows that $H_2(\rho_b)$ is also achievable which concludes the proof of Theorem~\ref{thm:UB2}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem~\ref{thm:UB3}}\label{sec:thm-UB3-proof}

Let $K = \sum_{i=1}^p X_i$. Then, for any pair $(U,\bX)$ such that $U \rw \bX \rw (\bY,\bZ)$, we have
\begin{align}
&I(U; \bY) - I(U;\bZ) \nonumber \\
 &= I(\bX; \bY) - I(\bX;\bZ) + I(\bX;\bZ|U)  - I(\bX;\bY | U) \\
%& = I(\bX; \bY| K) + I(K; \bY) -  I(\bX;\bZ|K) - I(K;\bZ) \nonumber \\
%&\quad + I(\bX;\bZ|U,K)   + I(K,\bZ|U) \nonumber \\
%& \quad - I(\bX;\bY | U,K) - I(K;\bY|U)\\
& \le I(\bX; \bY|K) - I(\bX;\bZ|K) \nonumber \\
&\quad + I(\bX;\bZ|U,K)  - I(\bX;\bY | U,K) + 2 \log p\\
& \le \max_{0 \le k \le p} \Delta(k) + 2 \log p%\Big[  I(\bX; \bY|K=k) - I(\bX;\bZ|K=k) \nonumber \\
%&\quad + I(\bX;\bZ|U,K=k)  - I(\bX;\bY | U,K=k)\Big] + 2 \log p
\end{align}
where
\begin{align*}
\Delta(k) &=  I(\bX; \bY|K=k) - I(\bX;\bZ|K=k) \nonumber \\
& \quad + I(\bX;\bZ|U,K=k)  - I(\bX;\bY | U,K=k).
\end{align*}

We now consider two cases. For the case $m_b \le k \le p$, we use the upper bound
\begin{align*}
\Delta(k) &\le  I(\bX;\bY|K=k) + I(\bX;\bZ|U,K=k)\\
&\le  I(\bX;\bY|K=k) + I(\bX;\bZ|K=k)
%&\le \max_{\bX \in \mathcal{X}_k^p} I(\bX;\bY) + \max_{\bX \in \mathcal{X}_k^p} I(\bX;\bZ)
\end{align*}
which follows from the non-negativity of mutual information and the data processing inequality. 
Following the steps outlined in the proofs of Theorems~\ref{thm:UB1} and \ref{thm:UB2} shows that
\begin{align}
\limsup_{p \rw \infty}  \max_{\bX \in \mathcal{X}_k^p\; : \; m_b \le k \le p}  {\textstyle \frac{1}{p}} \Delta(k) & \le \textstyle \frac{1}{2}  (\rho_b+\rho_e) \log e  \le \rho_b \log e
\end{align}
almost surely. (Note that this step does not require the symmetry assumption.)

%Now, let $k = \lfloor \kappa p \rfloor$. Using the bound
%\begin{align}
%\Delta(k) \le  \max_{\bX \in \mathcal{X}_k^p} I(\bX;\bY) + \max_{\bX \in \mathcal{X}_k^p} I(\bX;\bZ),
%\end{align}
%and results from Section~\ref{sec:thm-UB2-proof} shows that if $\kappa > \rho_b$, then
%\begin{align}
%\limsup_{p \rw \infty}{\textstyle \frac{1}{p}} \Delta(k) & \le \textstyle \frac{1}{2}  \rho_b + \frac{1}{2} \rho_e  \le \rho_b.
%\end{align}
Alternatively, for the case $0 \le k < m_b$, we use the bound
\begin{align*}
\Delta(k) \le H(\bX|\bZ,K=k) + H(\bX|\bY,K=k)
\end{align*}
which follows from the non-negativity of entropy and the fact that conditioning cannot increase entropy. Since $\bA_b$ is fully linearly independent almost surely, it follows from the proof of Theorem~\ref{thm:LB1} that $H(\bX|\bY,K=k)$ is equal to zero almost surely. To characterize the asymptotic behavior of the remaining term, $H(\bX|\bZ,K=k)$, we use the following lemma which is proved in Appendix \ref{sec:HXZ-proof}. 

% it follows from the proof of Theorem~\ref{thm:LB2} that $H(\bX|\bY,K=k)$ is equal to zero almost surely and thus
%\begin{align}
% \Delta(k) \le  H(\bX|\bZ, K =k).
%\end{align}
%To upper bound $H(\bX|\bZ,K=k)$ we use the following lemma whose proof is omitted due to space constraints. % which is proved in the appendix.

\begin{lemma}\label{lem:HXZ}
Suppose that $\bX$ is symmetric. If $0 \le k < m_b$ and $k/p \rw \kappa$ where $0 \le \kappa \le \rho_b$, then
%If $\bX$ is symmetric, then% where $k = \lceil \kappa \rho \rceil$, then
\begin{align}
&\limsup_{p \rw \infty}{\textstyle \frac{1}{p}} H(\bX|\bZ, K =k)  \le g(\kappa,\rho_e)
\end{align}
almost surely where 
\begin{align}
g(\kappa,\rho_e) =  H(X| W X + \sqrt{\kappa/\rho_e}V) \label{eq:lemHXZ}
\end{align}
and 
$X\sim\text{Bernoulli}(\kappa)$, $W \sim \mathcal{N}(0,1)$ and $V\sim \mathcal{N}(0,1)$ are independent random variables.
\end{lemma}

Noting that $g(\kappa,\rho_e)$ is nondecreasing in $\kappa$, we obtain the asymptotic upper bound
\begin{align}
\limsup_{p \rw \infty} C_s \le \max \big(g(\rho_b,\rho_e), \rho_b \big).
\end{align}
It can be verified numerically that this maximum occurs at $g(\rho_b,\rho_e)$ for all $\rho_b \in (0,1/2)$ which completes the proof of Theorem~\ref{thm:UB3}.

==> sections/results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Main Results}

Csiszar and Korner showed in \cite{csiszar} that the secrecy capacity of a discrete memoryless wiretap channel is given by
\begin{align} C_s = \max_{(U, \bX)} \big[{\textstyle \frac{1}{p} } I(U ;\bY) - {\textstyle \frac{1}{p} }I(U; \bZ)] \label{eq:CsThm}
\end{align}
where the auxiliary random variable $U$ satisfies the Markov chain relationship: $U \rw \bX \rw (\bY,\bZ)$. It can be verified that this is also the secrecy capacity when the channels have discrete inputs and continuous outputs (see e.g. \cite{liu07}).

In some special cases, the secrecy capacity can be computed easily from \eqref{eq:CsThm}. For example, if $A_b$ and $A_e$ correspond to the first $m_b$ and $m_e$ rows of the $p \times p$ identity matrix respectively, then it is straightforward to show that
\begin{align}
C_s%& = \max\left(\max_{\bX} {\textstyle \frac{1}{p} }I(\bX;\bY) -
%\max_{\bX}{\textstyle \frac{1}{p} } I(\bX; \bZ), 0\right)\\
& =
\begin{cases}
  \textstyle \frac{m_b}{p} - \frac{m_e}{p}, & \text{if $m_e< m_b$}\\
  0 & \text{if $m_e \ge m_b$}
  \end{cases} .
  \label{eq:CsIdentity}
\end{align}
In this case, the secrecy capacity happens to be the difference of the individual channel capacities; thus as $m_e$ approaches $m_b$ the secrecy capacity tends to zero. In the following sections we will develop bounds for a class of matrices inspired by compressed sensing. Interestingly, we will see that the secrecy behavior of these matrices differs greatly from the behavior shown in \eqref{eq:CsIdentity}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Lower Bounds}\label{sec:LB}

We say that a matrix $A\in \mathbb{R}^{m \times p}$ is {\em fully linearly independent} (FLI) if the span of each submatrix $\{A(\bx) \in \mathbb{R}^{m \times m-1} \; : \; \bx \in \mathcal{X}^p_{m-1}\}$ defines a unique linear subspace of $\mathbb{R}^m$. Examples of FLI matrices include the first $m$ rows of the $p \times p$ discrete cosine transform matrix or, with probability one, any matrix whose entries are drawn i.i.d.~from a continuous distribution. A counter example is given by the first $m$ rows of the $p\times p$ identity matrix.

Our first result, which is proved in~Section~\ref{sec:thm-LB1-proof}, gives a general lower bound on the secrecy capacity for any FLI matrices.

% provided that Bob's channel matrix has at least one more row than Eve's channel matrix. 

\begin{theorem}\label{thm:LB1}  Suppose that $A_b$ and $A_e$ are fully linearly independent. If $m_e < m_b$, then the secrecy capacity is lower bounded by
\begin{align}
C_s &\ge \textstyle \frac{1}{p}  \log{p \choose m_b -1} - \frac{1}{2p} \log \det(\frac{1}{p} A_e A_e^T) \nonumber\\
&+%{\textstyle \frac{1}{2p}}
 \sum_{\bx \in \mathcal{X}^p_{m_b-1}} \textstyle {\textstyle \frac{1}{ {p \choose m_b -1}2 p}} \log \det\left( \frac{1}{m_b-1}A_e(\bx) A_e(\bx)^T\right).  \label{eq:CsLB1}
\end{align}
\end{theorem}

%Note that the bound in Theorem~\ref{thm:LB1} applies only if the number of rows in Bob's channel matrix is strictly greater than the the number of rows in Eve's channel matrix. Otherwise, 

%Bob receives at least one more measurement than Eve does.  It is important to note that if the rows of $A_b$ are a subset of the rows of $A_e$ then no secret information can be transmitted. Thus, without further qualifications the only universal lower bound for the setting $m_e \ge m_b$ is $C_e \ge 0$.  

The lower bound in Theorem~\ref{thm:LB1} is derived by evaluating the right hand side of \eqref{eq:CsThm} when $\bX$ is distributed uniformly over the set $\mathcal{X}_{m_b-1}^p$. We note that the condition $m_e < m_b$ is necessary to obtain a nontrivial lower bound since the secrecy capacity may be equal to zero otherwise. 

%
% It can be verified that this lower bound is strictly positive. 

%It is important to note that if $m_e \ge m_b$ then the secrecy capacity may be equal to zero. 

%
%the inequality $m_e < m_b$ is necessary to obtain a non-trivial bound. In the case $m_e \ge m_b$, then it may be the case that 

%, without further qualifications, the best possible lower bound for the case $m_e \ge m_b$ is $C_e \ge 0$ since it may be the case that the ows of $A_b$ are a subsets of the rows of $A_e$.  

%

%It is important to note that the strict inequality $m_e < m_b$ is necessary to obtain a nontrivial lower bound. Otherwise, it

%the secrecy capacity can be equal to zero. This occurs, for example, if the rows of $A_b$ are a subsets of the rows of $A_e$.  

%is is straightforward to show that that secrecy capacity is equal to zero. Thus, Theorem~\ref{thm:LB3} shows that there is a {\em discontinuity} in the asymptotic secrecy capacity as a function of $\rho_e$. %One open question then, is what happens in setting where $m_b/m_e \rw 1$ with $m_e < m_b$. 


Unfortunately, the bound in Theorem~\ref{thm:LB1} is difficult to compute if $m_b$ and $p$ are large. One way to address this issue is to analyze the behavior for a random matrix (random matrices are denoted via boldface, uppercase letters). The following result is proved in~Section~\ref{sec:thm-LB2-proof}.

\begin{theorem}\label{thm:LB2}
Suppose that $A_b$ is fully linearly independent and $\bA_e$ is a random matrix whose elements are i.i.d.~$\mathcal{N}(0,1)$. If $m_e < m_b$ then the expectation of the secrecy capacity is lower bounded by
\begin{align}
\bE_{\bA_e}[ C_s ] &\ge  \textstyle \frac{1}{p}  \log{p \choose m_b -1} -  \frac{m_e}{2p}\log \big( \frac{m_b-1}{p}\big) \nonumber\\
& - {\textstyle \frac{ \log e}{2p}}  \sum_{i=1}^{m_e}\big[{ \textstyle \psi\left(\frac{p-i +1}{2} \right) - \psi\left(\frac{m_b -i}{2} \right) } \big]  \label{eq:LB2}
\end{align}
where $\psi(x) = \Gamma'(x)/\Gamma(x)$ is Euler's digamma function.
\end{theorem}

One benefit of Theorem~\ref{thm:LB2} is that the bound is independent of the realization of the matrix $\bA_e$ and can be analyzed directly. An illustration of the bound is shown in Figure~\ref{fig:IIDbounds_expectation} as a function of $m_e/p$ for various values of $p$ with $m_b/p$ held fixed. Remarkably, as $p$ becomes large, the lower bound in Theorem~\ref{thm:LB2} remains bounded away from zero for all values of $m_e$ strictly less than $m_b$. This behavior is in stark contrast to the secrecy capacity shown in \eqref{eq:CsIdentity}. 

%One intuitive explanation for why occurs is provided in Section~\ref{sec:conclusion}.

%This means that the secrecy capacity does not tend to zero as the capacity of eavesdropper tends to capacity of the main channel.
%The key reason for this difference is the the FLI matrices 


\begin{figure}
\centering
\psfrag{xlabel}[]{ $m_e/p$}
\psfrag{ylabel}[B][bt][1][0]{Secrecy Capacity $C_s$}
\psfrag{title}{}
\includegraphics[width=.9 \columnwidth]{figures/bounds_exp.eps}
\caption{\label{fig:IIDbounds_expectation} Illustration of the lower bound in Theorem~\ref{thm:LB2} on the expected secrecy capacity $\bE_{\bA_e}[C_s]$ as a function of $m_e$ for various values of $p$ when $A_b$ is fully linearly independent, $\bA_e$ is a random matrix whose elements are i.i.d.~$\mathcal{N}(0,1)$, and $m_b/p = 0.2$.} 
%Bounds on the asymptotic (normalized) secrecy capacity $C_s$ of the multiplicative Gaussian wiretap channel as a function of $\rho_e$ when $\rho_b=0.2$ and $\bA_b$ and $\bA_e$ are random matrices whose elements are i.i.d.~$\mathcal{N}(0,1)$.}
\end{figure}



One shortcoming of Theorem~\ref{thm:LB2}, is that the bound holds only in expectation, and it is possible that it is violated for a constant fraction of matrices $\bA_e$. The next result, which is proved in~Section~\ref{sec:thm-LB3-proof}, shows that, in the asymptotic setting, the limit of the bound $\eqref{eq:LB2}$ holds for almost every realization of $\bA_e$. We use the notation $\{A^{(p)} \in \mathbb{R}^{m^{(p)} \times p}\}$ to denote a sequence of matrices indexed by the number of columns $p$. %$m^{(p)} \times p$ matrices where $m^{(p)}$ is a sequence of integers.
%The next result says that if $p,m_b,m_e$ are large and $\bA_e$ has i.i.d.~elements, then the lower bound will hold for almost every realizati on of $\bA_e$.

\begin{theorem}\label{thm:LB3}
Suppose that $\{A_b^{(p)} \in \mathbb{R}^{m_b^{(p)} \times p}\}$ is a sequence of linearly independent matrices and $\{\bA_e^{(p)}\in \mathbb{R}^{m_e^{(p)}} \times p\}$ is a sequence of random matrices whose elements are i.i.d.~$\mathcal{N}(0,1)$.  If $m_e^{(p)} > m_b^{(p)}$ and $m_b^{(p)} / p \rw \rho_b$ and $m_e^{(p)}/p \rw \rho_e$ as $p \rw \infty$ where $0\le \rho_e \le \rho_b \le 1/2$, then the asymptotic secrecy capacity is lower bounded by
\begin{align}
\liminf_{p \rw \infty} C_s \ge H_2(\rho_b) - \textstyle \frac{1}{2}\Big [ &(1 - \rho_e) \log\big(\textstyle\frac{1} {1 - \rho_e} \big)\nonumber \\
&- (\rho_b - \rho_e) \log\big(\textstyle \frac{\rho_b}{\rho_b - \rho_e}\big) \Big]
\end{align}
almost surely.
\end{theorem}

Theorem~\ref{thm:LB3} provides a concise characterization of the lower bound in the asymptotic setting. The bound is illustrated in  Figure~\ref{fig:IIDbounds_expectation} in the case $p= \infty$. Since the secrecy capacity can be equal to zero if $m_e^{(p)}=m_b^{(p)}$, Theorem~\ref{thm:LB3} shows that there is a {\em discontinuity} in the asymptotic secrecy capacity as a function of $\rho_e$. 

%In other words, if we define $\mathcal{C}_s(\rho_b,\rho_e) = \lim_{p \rw \infty} C_s$ to be the asymptotic secrecy rate when $m_b^{(p)} = \lfloor \rho_b\, p\rfloor$ and $m_e^{(p)} = \lfloor \rho_e\, p\rfloor$ then
%\begin{align}
%\lim_{\rho_e \uparrow \rho_b} \mathcal{C}_s(\rho_b,\rho_e) % &\ge H_2(\rho_b) - \textstyle \frac{1}{2} (1-\rho_b) \log \big( \frac{1}{1-\rho_b})\\
%& \ne \mathcal{C}_s(\rho_b,\rho_b).
%\end{align}

% the limit as $m^{(p)}_e/m^{(p)}_b$ approaches 1 from below does not equal the limit as $m^{(p)}_e/m^{(p)}_b$ approaches 1 from the above. 

%What is remarkable about the behavior shown in Theorem~\ref{thm:LB3} is that the lower bound is nearly equal to $H(\rho_b)$ even if $\rho_e$ is equal to $\rho_b$. This means that the secrecy capacity does not tend to zero as the capacity of eavesdropper tends to capacity of the main channel.

%
%It is important to note that Theorem~\ref{thm:LB3} requires the strict inequality $m_b > m_e$. If $m_b = m_e$, then is is straightforward to show that that secrecy capacity is equal to zero. Thus, Theorem~\ref{thm:LB3} shows that there is a {\em discontinuity} in the asymptotic secrecy capacity as a function of $\rho_e$. %One open question then, is what happens in setting where $m_b/m_e \rw 1$ with $m_e < m_b$. 

\subsection{Upper Bounds via Channel Capacity}\label{sec:UB}

This section considers the capacity of Bob's channel which is denoted $C_b$. We note that this capacity gives us an upper bound on the secrecy capacity.

Upper bounding the capacity is more technically challenging than lower bounding the secrecy capacity, since the optimal distribution on $\bX$ may depend nontrivially on channel matrix $A_b$. The following result, which is proved in~Section~\ref{sec:thm-UB1-proof}, serves as a starting point.

\begin{theorem}\label{thm:UB1} If $A_b$ is fully linearly independent, then the channel capacity of Bob's channel is upper bounded by
\begin{align}
%C_{b}& \le  {\textstyle \frac{1}{p}} \max\big ( f_1(m_b,p), f_2(m_b,p) \big) + {\textstyle  \frac{\log p}{p}}
%
C_{b} &\le {\textstyle \frac{1}{p}} \max\big ( {\textstyle  \log{p \choose m_b-1}} ,  \max_{m_b \le k \le p} \tilde{c}(k) \big) + {\textstyle  \frac{\log p}{p}}\label{eq:thm:UB1}
\end{align}
where
\begin{align}
%f_1(m_b,p) &= \max_{0\le k < m_b} {\textstyle  \log{p \choose k}}\\
%f_2(m_b,p) & ={\textstyle \frac{1}{2}} \Big[ \max_{1 \le i \le p} \textstyle {m_b} \log\big(\textstyle \frac{1}{m_b} \| A_b(i)\|^2 \big)  \nonumber\\
%&\quad -  \max_{m_b \le k \le p} \max_{\bx \in \mathcal{X}_k^p} \textstyle \log \det\big( \frac{1}{k} A_b(\bx) A_b(\bx)^T\big)\Big].\label{eq:f2}
\tilde{c}(k)  &= \max_{1 \le i \le p} \textstyle \frac{m_b}{2} \log\big(\textstyle \frac{1}{m_b} \| A_b(i)\|^2 \big)  \nonumber\\
&\quad -  \max_{\bx \in \mathcal{X}_k^p} \textstyle \frac{1}{2} \log \det( \frac{1}{k} A_b(\bx) A_b(\bx)^T).\label{eq:Ctilde}
\end{align}
\end{theorem}

Although it is tempting to consider the expectation of \eqref{eq:thm:UB1} with respect to a random matrix (as we did for Theorem~\ref{thm:LB2}), this is difficult since the maximization in \eqref{eq:Ctilde} occurs inside the expectation.

Our next result, which is proved in~Section~\ref{sec:thm-UB2-proof}, leverages the strong concentration properties of the Gaussian distribution to characterize the asymptotic capacity for Gaussian matrices.
\begin{theorem}\label{thm:UB2}
Suppose that $\{\bA_b^{(p)} \in \mathbb{R}^{m_b^{(p)} \times p} \}$ is a sequence of random matrices whose elements are i.i.d.~$\mathcal{N}(0,1)$.  If $m_b^{(p)}/p \rw  \rho_b$ where $0 < \rho_b \le 1/2$, then the asymptotic channel capacity of Bob's channel is given by
\begin{align}
\lim_{p \rw \infty} C_b = H_2(\rho_b)
%\begin{cases}
%H_2(\rho_b), & \text{\normalfont if $0 \le \rho_b <1/2$}\\
%H_2(\frac{1}{2}), & \text{\normalfont if $1/2 \le \rho_b \le 1$}
%\end{cases}
\end{align}
almost surely.
\end{theorem}

Theorem~\ref{thm:UB2} shows that the strategy used in our lower bounds, namely choosing $\bX$ uniformly over $\mathcal{X}_{m_b-1}^p$ achieves the capacity of Bob's channel in the asymptotic setting. What is remarkable is that for this same input distribution, Eve learns very little about what is being sent, even if her channel matrix is equal to the first $m_e$ rows of Bob's channel matrix. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Improved Upper Bound for a Restricted Setting}\label{sec:UB2}

We say that the distribution is {\em symmetric} if $\Pr[\bX=\bx]= \Pr[\bX=\tilde{\bx}]$ for all $\bx,\tilde{\bx}$ such that $\sum_{i=1}^p x_i=\sum_{i=1}^p \tilde{x}_i$. The following result is proved in Section~\ref{sec:thm-UB3-proof}.

\begin{theorem}\label{thm:UB3}
Suppose that $\{\bA_b^{(p)}\in \mathbb{R}^{m_b^{(p)} \times p}\}$ and $\{\bA_e^{(p)}\in \mathbb{R}^{m_e^{(p)} \times p}\}$ are sequences of random matrices whose elements are i.i.d.~$\mathcal{N}(0,1)$. If $m_b^{(p)} > m_e^{(p)}$ and  $m_b^{(p)} / p \rw \rho_b$, and $m_e^{(p)}/p \rw \rho_e$ where $0\le \rho_e \le \rho_b \le 1/2$, and if Alice is restricted to use coding strategies that induce a symmetric distribution on $\bX$, then the asymptotic secrecy capacity is upper bounded by
\begin{align}
\limsup_{p \rw \infty} C_s \le  H(X | W X + {\textstyle \sqrt{{\rho_b/\rho_e}}} V)
\end{align}
almost surely where $X\sim\text{Bernoulli}(\rho_b)$, $W \sim \mathcal{N}(0,1)$ and $V\sim \mathcal{N}(0,1)$ are independent random variables.
\end{theorem}

The bound in Theorem \ref{thm:UB3} is strictly less than the channel capacity $H_2(\rho_b)$ for all $\rho_e >0$, and can be computed easily using numerical integration. We suspect that this result also holds without the symmetry restriction on $\bX$.


%\section{Discussion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Illustration of Bounds}\label{sec:figs}

The bounds on the asymptotic secrecy capacity given in Theorems~\ref{thm:LB3}, \ref{thm:UB2}, are \ref{thm:UB3} and illustrated in Fig. \ref{fig:IIDbounds} as a function of the size parameter $\rho_e$ of the eavesdropper channel. The bounds correspond to the setting where the elements of the matrices are i.i.d.~Gaussian. Note that the lower bound on the secrecy capacity is nearly equal to that of the main channel for all $\rho_e < \rho_b$.

For comparison, the secrecy capacity for the special case where $A_b$ and $A_e$ correspond to the first rows of the $p \times p$ identity matrix are shown in Fig. \ref{fig:Ibounds}. In this case, the secrecy capacity is equal to the difference of the main channel capacity and eavesdropper capacity.


\begin{figure}
\centering
\psfrag{xlabel}[]{ $\rho_e$}
\psfrag{ylabel}[B][bt][1][0]{Secrecy Capacity $C_s$}
\psfrag{title}{}
\includegraphics[width=.9 \columnwidth]{figures/bounds1.eps}
\caption{\label{fig:IIDbounds}Bounds on the asymptotic (normalized) secrecy capacity $C_s$ of the multiplicative Gaussian wiretap channel as a function of $\rho_e$ when $\rho_b=0.2$ and $\bA_b$ and $\bA_e$ are random matrices whose elements are i.i.d.~$\mathcal{N}(0,1)$.}
\end{figure}


\begin{figure}
\centering
\psfrag{xlabel}[]{ $\rho_e$}
\psfrag{ylabel}[B][bt][1][0]{Secrecy Capacity $C_s$}
\psfrag{title}{}
\includegraphics[width=0.9 \columnwidth]{figures/bounds2.eps}
\caption{\label{fig:Ibounds}The (normalized) secrecy capacity $C_s$ of the multiplicative Gaussian wiretap channel as  a function of $\rho_e$ when $\rho_b=0.2$ and $A_b$ and $A_e$ correspond to the first rows of the identity matrix.}
\end{figure}


%\section{Intuitive Explanation of Behavior}


